iCap: Interactive Image Captioning with Predictive Text

In this paper we study a brand new topic of interactive image captioning with human in the loop. Different from automated image captioning where a given test image is the sole input in the inference stage, we have access to both the test image and a sequence of (incomplete) user-input sentences in the interactive scenario. We formulate the problem as Visually Conditioned Sentence Completion (VCSC). For VCSC, we propose asynchronous bidirectional decoding for image caption completion (ABD-Cap). With ABD-Cap as the core module, we build iCap, a web-based interactive image captioning system capable of predicting new text with respect to live input from a user. A number of experiments covering both automated evaluations and real user studies show the viability of our proposals.

==> performance-table.tex <==
\begin{table*}[t]\centering
    \caption{Performance of the Proposed Image Captioning Model on Character-level and Word-level COCO-CN Dataset.}
    \ra{1.3}
    \label{tab:caption-performance}
    \begin{tabular}{@{}lrrrrrcrrrrrc@{}}
        \toprule
        & \multicolumn{5}{c}{Character-level}  & \phantom{abc} & \multicolumn{5}{c}{Word-level} \\
        \cmidrule{2-6} \cmidrule{8-12}
        Method                      & Bleu\_4  & METEOR  & ROUGE\_L & CIDEr & OOV  && Bleu\_4  & METEOR  & ROUGE\_L & CIDEr & OOV  \\
        \midrule
        Show and Tell               & 24.0     & 27.1    & 47.8     & 70.6  & 0    && 25.5     & 27.4    & 48.4     & 72.4  & 53   \\
        Show and Tell (Backward)    & 23.0     & 26.6    & 47.0     & 68.2  & 0    && 23.9     & 27.0    & 48.2     & 71.5  & 73   \\
        \midrule
        Show and Tell (ABD)         & 24.4     & 27.6    & 48.3     & 71.7  & 0    && 26.0     & 27.3    & 48.6     & 73.7  & 105  \\
        \bottomrule
    \end{tabular}
\end{table*}
